Near-Optimal Packet Scheduling in Multihop Networks with End-to-End Deadline Constraints

Scheduling packets with end-to-end deadline constraints in multihop networks is an important problem that has been notoriously difficult to tackle. Recently, there has been progress on this problem in the worst-case traffic setting, with the objective of maximizing the number of packets delivered within their deadlines. Specifically, the proposed algorithms were shown to achieve $\Omega(1/\log(L))$ fraction of the optimal objective value if the minimum link capacity in the network is $C_{\min}=\Omega(\log (L))$, where $L$ is the maximum length of a packet's route in the network (which is bounded by the packet's maximum deadline). However, such guarantees can be quite pessimistic due to the strict worst-case traffic assumption and may not accurately reflect real-world settings. In this work, we aim to address this limitation by exploring whether it is possible to design algorithms that achieve a constant fraction of the optimal value while relaxing the worst-case traffic assumption. We provide a positive answer by demonstrating that in stochastic traffic settings, such as i.i.d. packet arrivals, near-optimal, $(1-\epsilon)$-approximation algorithms can be designed if $C_{\min} = \Omega\big(\frac{\log (L/\epsilon) } {\epsilon^2}\big)$. To the best of our knowledge, this is the first result that shows this problem can be solved near-optimally under nontrivial assumptions on traffic and link capacity. We further present extended simulations using real network traces with non-stationary traffic, which demonstrate that our algorithms outperform worst-case-based algorithms in practical settings.

==> Model.tex <==
\section{Model and Definitions}\label{sec:model}


==> nice-diagram.tex <==
\begin{tikzpicture}[
    every path/.style = {},
    every node/.append style = {font=\sffamily}
  ]
  \begin{scope}
    \shade[right color=green, left color=white, opacity=0.7]
      (-0.5,-0.5) rectangle (0,6.5);
    \node[rotate=90, above] at (0,3) {Non-Negative Gold};
    \shade[top color=yellow, bottom color=white, opacity=0.7]
      (-0.5,-0.5) rectangle (8.5,0);
    \node[below] at (4,0) {Non-Negative Bills};
    \shade[left color=red, bottom color=red, right color=white, opacity=0.5]
      (-0.5,5.5) -- (8.5,3) -- (8.5,6.5) -- (-0.5,6.5) -- cycle;
    \path (-0.5,5.5) -- node[pos=0.23, sloped, above] {Volume Constraint}
      (8.5,3);
    \shade[left color=orange, right color=white, opacity=0.5]
      (5,6.5) -- (8.5,6.5) -- (8.5,0) -- (5,0) -- cycle;
    \path (5.5,5.3) -- node[pos=0.3, sloped, above] {NP-Complete} (10,5.3);
    \node[text width=7em, align=center] at (2,2)
      {Feasible Region of the Linear Relaxation};
    \draw[->] (-0.5,0) -- (8.5,0) node[below] {Complexity};
    \draw[->] (0,-0.5) -- (0,6.5) node[above] {Efficiency Ratio};
    \path[clip] (-0.5,-0.5) rectangle (8.5,6.5);
    \end{scope}
\end{tikzpicture}


